Design Initiative for a 10 TeV pCM Wakefield Collider

This document outlines a community-driven Design Study for a 10 TeV pCM Wakefield Accelerator Collider. The 2020 ESPP Report emphasized the need for Advanced Accelerator R\&D, and the 2023 P5 Report calls for the ``delivery of an end-to-end design concept, including cost scales, with self-consistent parameters throughout." This Design Study leverages recent experimental and theoretical progress resulting from a global R\&D program in order to deliver a unified, 10 TeV Wakefield Collider concept. Wakefield Accelerators provide ultra-high accelerating gradients which enables an upgrade path that will extend the reach of Linear Colliders beyond the electroweak scale. Here, we describe the organization of the Design Study including timeline and deliverables, and we detail the requirements and challenges on the path to a 10 TeV Wakefield Collider.

==> synergies.tex <==
The 10 TeV Wakefield Collider Design Study must solve a number of challenges in order to create a viable path towards a future collider. The Design Study is required to innovate in order to address technical risks. Some of these innovations will be necessary for a 10 TeV Collider, but also beneficial to nearer-term machines. Although our study is still in its early stages, we have already identified several tasks which will benefit Higgs Factory design and optimization. These include: 1) High-Performance Computing (HPC) Particle-in-Cell (PIC) codes for modeling beam-beam interactions, 2) Laser-based collimation systems~\cite{Zimmermann1999}, 3) Non-intercepting diagnostics for ultra-intense beams.

The Design Study has natural synergies with all future Linear Collider Higgs Factories as a long term upgrade to such a machine. The upgrade path for a Linear Collider Facility is detailed in the LC Visions document~\cite{LCVisions:2025}. The 10 TeV Wakefield Collider Design Study both complements and benefits from on-going design efforts including ALEGRO~\cite{ALEGRO:2019}, HALHF~\cite{foster2023hybrid}, ALIVE~\cite{Farmer_2024}, XCC~\cite{XCC:2023}, the Muon Collider~\cite{MC:2024}.


% While the 10 TeV Design Study has clear aims to provide an end-to-end concept of a future collider, there are ample areas of overlap between the R\&D needed for 10 TeV collisions and R\&D that will benefit near-term Higgs Factories.
% \begin{itemize}
%     \item Beam-beam codes
%     \item laser collimation
%     \item diagnostics
%     \item detector test beams
%     \item near term applications
%     \item LC Upgrade
% \end{itemize}
